Unsupervised Discretization by Two-dimensional MDL-based Histogram

Unsupervised discretization is a crucial step in many knowledge discovery tasks. The state-of-the-art method for one-dimensional data infers locally adaptive histograms using the minimum description length (MDL) principle, but the multi-dimensional case is far less studied: current methods consider the dimensions one at a time (if not independently), which result in discretizations based on rectangular cells of adaptive size. Unfortunately, this approach is unable to adequately characterize dependencies among dimensions and/or results in discretizations consisting of more cells (or bins) than is desirable. To address this problem, we propose an expressive model class that allows for far more flexible partitions of two-dimensional data. We extend the state of the art for the one-dimensional case to obtain a model selection problem based on the normalized maximum likelihood, a form of refined MDL. As the flexibility of our model class comes at the cost of a vast search space, we introduce a heuristic algorithm, named PALM, which Partitions each dimension ALternately and then Merges neighboring regions, all using the MDL principle. Experiments on synthetic data show that PALM 1) accurately reveals ground truth partitions that are within the model class (i.e., the search space), given a large enough sample size; 2) approximates well a wide range of partitions outside the model class; 3) converges, in contrast to the state-of-the-art multivariate discretization method IPD. Finally, we apply our algorithm to three spatial datasets, and we demonstrate that, compared to kernel density estimation (KDE), our algorithm not only reveals more detailed density changes, but also fits unseen data better, as measured by the log-likelihood.

==> exp1_table_MISE_for_loss_outliers.tex <==
% latex table generated in R 3.4.4 by xtable 1.8-4 package
% Tue Oct  1 11:54:11 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrr}
  \hline
%sample size & MISE for subgroup: $L_{lr} > 1$ & MISE for subgroup: $L_{tr} > 1$ & overall MISE \\ 
Sample size & MISE for subgroup: $L_{tr} > 1$ & overall MISE \\
\hline
 100,000 & 0.00148 & 0.00148 \\ 
  300,000 & 0.00055 & 0.00074 \\ 
  500,000 & 0.00051 & 0.00065 \\ 
  700,000 & 0.00019 & 0.00069 \\ 
  1,000,000 & 0.00023 & 0.00058 \\ 
  3,000,000 &  0.00017 & 0.00055 \\ 
  5,000,000 & 0.00006 & 0.00051 \\
   \hline
\end{tabular}
\caption{The average MISE of data in the subgroup whose $L_{tr} > 1$, and the overal mean of MISE. We show that, when PALM fails to identify part of the true partitions, the learned histogram model still estimates the probability density accurately. The only explanation for these cases is that, some neighbouring sub-regions in the true partitions have very similar ``true" $f_j$ defined in equation (\ref{eq25}), and PALM fails to identity line segments that partition these neighbouring sub-regions.}
\end{table}

